Cosmic Dragons: A Two-Component Mixture Model of COSMOS Galaxies

Using the photometric population prediction method {\bf Red Dragon}, we characterize the Red Sequence (RS) and Blue Cloud (BC) of DES galaxies in the COSMOS field. Red Dragon (RD) uses a redshift-evolving, error-corrected Gaussian mixture model to detail the distribution of photometric colors, smoothly parameterizing the two populations with relative weights, mean colors, intrinsic scatters, and inter-color correlations. This resulting fit of RS and BC yields RS membership probabilities $P_{\rm RS}$ for each galaxy. Even when training on only DES main bands $griz$, RD selects the quiescent population (defined here as galaxies with $\lg {\rm sSFR \cdot yr} < -11$) with $\gtrsim 90\%$ balanced accuracy out to $z=2$; augmenting with extended photometry from VIRCAM improves this accuracy to $\sim 95\%$ out to $z=3$. We measure redshift evolution of sSFR and galactic age in several stellar mass bins, finding that the BC is consistently more star-forming (by $\gtrsim 1~{\rm dex}$) and typically younger (by $\gtrsim 1~{\rm Gyr}$) than the RS (up to $z \sim 1.4$). This characterization of both RS and BC as functions of redshift and stellar mass improves our understanding of both populations and opens the door to more precise galaxy population characterization in future deep optical and IR systems.

==> appendices/nix_7Dv3D.tex <==

\iffalse
%  %  %  %  %  %  %  %  %  %  %  %  %  %  %  %
\subsection{Difference in selection between extended photometry and DES main bands} \label{sec:7D_vs_3D} 
% Slxn acc for 3D vs 7D

The difference in selection between dragons trained on DES main bands $griz$ and dragons trained on the extended photometry $ugriz + JHK_{\rm s}$ raises the question of mutual compatibility: To what accuracy can a dragon trained on $griz$ bands alone select RS galaxies as defined by a dragon trained on the extended photometry? 


\wm{TODO: plot bACC(z) for the three bins, with 7D as `truth'.} 

\begin{figure}\centering
  \includegraphics [width=\linewidth] {figs/bACC_7D_3D}
  \caption[bACC of DES main bands vs extended photometry]{
    Selection accuracy of using DES main bands ($griz$) alone, as compared to the extended photometry sample ($ugriz + JHK_{\rm s}$). 
    \textcolor{red}{[currently only for middle mass bin; preliminary placeholder result.]} 
    Looks like it's roughly 90\% except near the transition redshifts. 
  }
  \label{fig:7D_vs_3D}
\end{figure}

Note: bACC between bootstrap runs is typically $(97 \pm 1)\%$, so that's an effective maximum expected bACC here. Can't really expect bACC to be $\gtrsim 95\%$ when that's only barely the case between bootstraps. 
\fi 

